JYVA at BeTraC: Audio-Based Medical Note Generation with SOAP Section-Specific Queries

We present our submission to the Beyond Transcription Challenge (BeTraC) on medical note generation from doctor-patient audio conversations. We propose a section-aware approach based on Qwen2.5-Omni-3B, in which a lightweight Q-Former learns SOAP section-specific queries to extract compact clinical representations from speech. In the lightweight track, our system ranks fourth and substantially outperforms the challenge baseline, achieving a Concept F1 of 0.5005 on the official test set. The organizers' analysis and our heuristic evaluation suggest improved robustness to hallucinations, and better stability under difficult audio conditions. These results show that explicitly modeling SOAP structure through section-specific queries is an effective way to improve the faithfulness and reliability of audio-based medical note generation.

==> figures/system_overview.tex <==



\begin{figure*}[!ht]
\centering
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[x=1cm,y=1cm]

% ---------------------------------------------------------------------------
% Background stage frames
% ---------------------------------------------------------------------------
\begin{scope}[on background layer]
  \node[stageFrame, minimum width=17.9cm, minimum height=5.45cm, anchor=north west]
    (stage1box) at (-0.15,9.75) {};
  \node[stageFrame, minimum width=17.9cm, minimum height=2.95cm, anchor=north west]
    (stage2box) at (-0.15,3.95) {};
\end{scope}

\node[anchor=west, font=\bfseries\small] at (-0.05,10.15)
  {Two-stage section-aware Q-Former adaptation of Qwen2.5-Omni for speech-to-SOAP summarization};

% ---------------------------------------------------------------------------
% Stage 1: expanded Q-Former pretraining
% ---------------------------------------------------------------------------
\node[anchor=west, font=\bfseries] at (0.15,9.45)
  {Stage 1: Clinical Q-Former pretraining};

\node[anchor=west, note] at (0.15,9.18)
  {Native Qwen audio projector removed; speech tower frozen; Q-Former and thinker LoRA trained with global, concept, and section-specific losses.};

\node[frozen, minimum width=16mm] (audio1) at (0.80,8.12) {Dialogue\\audio};
\node[frozen, minimum width=20mm] (tower1) at (2.55,8.12) {Frozen\\speech tower};
\node[frozen, minimum width=20mm] (emb1)   at (4.30,8.12) {Speech\\embeddings};

\draw[flow] (audio1) -- (tower1);
\draw[flow] (tower1) -- (emb1);

% Q-Former internal view
\node[trainable, minimum width=6.0cm, minimum height=3.65cm]
  (qformer1) at (7.95,7.25) {};

\node[anchor=north, font=\bfseries\scriptsize] at (qformer1.north)
  {Trainable clinical Q-Former adapter};

\node[anchor=north, note] at ($(qformer1.north)+(0,-0.28)$)
  {96 learned queries; 2 transformer layers; cross-attention to speech};

% Query groups at input
\node[qrowS]  (qs0)  at (5.55,7.90) {$Q_S$\\32 Subjective};
\node[qrowO]  (qo0)  at (5.55,7.20) {$Q_O$\\32 Objective};
\node[qrowAP] (qap0) at (5.55,6.50) {$Q_{AP}$\\32 A\&P};

\node[anchor=south, note] at (5.55,8.30)
  {learned query groups};

% Two Q-Former blocks
\node[block] (blk1) at (7.25,7.20) {};
\node[font=\bfseries\tiny] at ($(blk1.north)+(0,-0.20)$)
  {Q-Former block 1};
\node[micro] (b1sa) at (7.25,7.78) {query\\self-attn};
\node[micro] (b1ca) at (7.25,7.18) {cross-attn\\to speech};
\node[micro] (b1ff) at (7.25,6.58) {FFN};

\node[block] (blk2) at (8.80,7.20) {};
\node[font=\bfseries\tiny] at ($(blk2.north)+(0,-0.20)$)
  {Q-Former block 2};
\node[micro] (b2sa) at (8.80,7.78) {query\\self-attn};
\node[micro] (b2ca) at (8.80,7.18) {cross-attn\\to speech};
\node[micro] (b2ff) at (8.80,6.58) {FFN};

% Output tokens by group
\node[qrowS]  (zs)  at (10.35,7.90) {$Z_S$\\S tokens};
\node[qrowO]  (zo)  at (10.35,7.20) {$Z_O$\\O tokens};
\node[qrowAP] (zap) at (10.35,6.50) {$Z_{AP}$\\A\&P tokens};

\node[anchor=south, note] at (10.35,8.30)
  {task-oriented outputs};

% Query paths inside the Q-Former
\draw[sFlow]  (qs0.east)  -- ($(blk1.west)+(0,0.45)$);
\draw[oFlow]  (qo0.east)  -- (blk1.west);
\draw[apFlow] (qap0.east) -- ($(blk1.west)+(0,-0.45)$);

\draw[sFlow]  ($(blk1.east)+(0,0.45)$) -- ($(blk2.west)+(0,0.45)$);
\draw[oFlow]  (blk1.east) -- (blk2.west);
\draw[apFlow] ($(blk1.east)+(0,-0.45)$) -- ($(blk2.west)+(0,-0.45)$);

\draw[sFlow]  ($(blk2.east)+(0,0.45)$) -- (zs.west);
\draw[oFlow]  (blk2.east) -- (zo.west);
\draw[apFlow] ($(blk2.east)+(0,-0.45)$) -- (zap.west);

% Cross-attention from audio embeddings to Q-Former blocks
\coordinate (kv) at (5.15,8.80);
\draw[flow, dashed] (emb1.east) -- ++(0.30,0) |-
  node[pos=.18, above, note] {cross-attention $K,V$} (kv);
\draw[flow, dashed] (kv) -- (b1ca.north west);
\draw[flow, dashed] (kv) -- (b2ca.north west);

% Thinker with LoRA in Stage 1
\node[lora, minimum width=2.15cm, minimum height=3.20cm]
  (think1) at (12.35,7.20) {};

\node[anchor=north, font=\bfseries\scriptsize] at (think1.north)
  {Thinker};

\node[anchor=north, note] at ($(think1.north)+(0,-0.30)$)
  {decoder-only LLM\\+ LoRA};

\node[box, fill=white, minimum width=15mm, minimum height=4.5mm, inner sep=1.2pt]
  at (12.35,7.95) {layers $1{\ldots}m$};

\node[box, fill=white, minimum width=15mm, minimum height=4.5mm, inner sep=1.2pt]
  at (12.35,7.20) {layers $m{+}1{\ldots}n$};

\node[box, fill=white, minimum width=15mm, minimum height=4.5mm, inner sep=1.2pt]
  at (12.35,6.45) {LM head};

% Colored entry/exit ports through the thinker
\coordinate (tinS)   at ($(think1.west)+(0,0.70)$);
\coordinate (tinO)   at ($(think1.west)+(0,0.00)$);
\coordinate (tinAP)  at ($(think1.west)+(0,-0.70)$);

\coordinate (toutS)  at ($(think1.east)+(0,0.70)$);
\coordinate (toutO)  at ($(think1.east)+(0,0.00)$);
\coordinate (toutAP) at ($(think1.east)+(0,-0.70)$);

\draw[sFlow]  (zs.east)  -- node[above, note, text=sColor] {S-token slice} (tinS);
\draw[oFlow]  (zo.east)  -- node[above, note, text=oColor] {O-token slice} (tinO);
\draw[apFlow] (zap.east) -- node[below, note, text=apColor] {A\&P-token slice} (tinAP);

% Losses
\node[loss, minimum width=21mm] (lossSOAP) at (15.10,8.65)
  {$\mathcal{L}_{\mathrm{SOAP}}$\\full SOAP note};

\node[smallloss, draw=sColor, text=sColor, fill=sColor!10] (lossS) at (15.10,7.90)
  {$\mathcal{L}_{S}$\\Subjective};

\node[smallloss, draw=oColor, text=oColor, fill=oColor!10] (lossO) at (15.10,7.20)
  {$\mathcal{L}_{O}$\\Objective};

\node[smallloss, draw=apColor, text=apColor, fill=apColor!12] (lossAP) at (15.10,6.50)
  {$\mathcal{L}_{AP}$\\Assessment/Plan};

\node[loss, draw=conceptColor, text=conceptColor, fill=conceptColor!10, minimum width=21mm]
  (lossConcept) at (15.10,5.65)
  {$\mathcal{L}_{\mathrm{concept}}$\\medical concepts};

\draw[flow] (think1.east) -- ++(0.30,0) |- (lossSOAP.west);
\draw[sFlow]  (toutS)  -- (lossS.west);
\draw[oFlow]  (toutO)  -- (lossO.west);
\draw[apFlow] (toutAP) -- (lossAP.west);
\draw[conceptFlow] (think1.east) -- ++(0.40,0) |- (lossConcept.west);

\node[anchor=west, note] at (13.55,8.18)
  {shared thinker,\\separate targets};

\draw[decorate, decoration={brace, amplitude=3pt}, draw=darkLine!70]
  (16.25,8.94) -- node[right=3pt, note] {Stage-1 supervision} (16.25,5.35);

% ---------------------------------------------------------------------------
% Stage 2: SOAP adaptation with native pathway restored
% ---------------------------------------------------------------------------
\node[anchor=west, font=\bfseries] at (0.15,3.68)
  {Stage 2: SOAP adaptation with native audio pathway restored};

\node[anchor=west, note] at (0.15,3.42)
  {Stage-1 Q-Former frozen; native audio projector restored; only a new thinker LoRA is trained.};

\node[frozen, minimum width=16mm] (audio2) at (0.80,2.45)
  {Dialogue\\audio};

\node[frozen, minimum width=20mm] (tower2) at (2.55,2.45)
  {Frozen\\speech tower};

\node[frozen, minimum width=21mm] (proj2) at (4.70,2.95)
  {Frozen native\\Qwen projector};

\node[trainable, minimum width=21mm, fill=trainFill!75] (qf2) at (4.70,1.90)
  {Frozen Stage-1\\Q-Former};

\node[loss, minimum width=28mm] (concat2) at (7.20,2.45)
  {Concatenate audio prefix\\\textbf{Q-Former tokens first}\\+ native audio tokens};

\node[lora, minimum width=20mm] (think2) at (9.90,2.45)
  {Thinker\\LoRA only};

\node[loss, minimum width=16mm, fill=lossFill!70] (soap2) at (11.95,2.45)
  {SOAP\\note};

\node[loss, minimum width=18mm] (loss2) at (14.00,2.45)
  {$\mathcal{L}_{\mathrm{SOAP}}$\\only};

\draw[flow] (audio2) -- (tower2);

\draw[flow] (tower2.east) -- ++(0.45,0) |-
  node[pos=.70, above, note] {native tokens} (proj2.west);

\draw[flow] (tower2.east) -- ++(0.45,0) |-
  node[pos=.70, below, note] {speech embeddings} (qf2.west);

\draw[flow] (proj2.east) --
  node[above, note] {projected audio} (concat2.west |- proj2.east);

\draw[oFlow] (qf2.east) --
  node[below, note, text=oColor] {96 clinical tokens} (concat2.west |- qf2.east);

\draw[flow] (concat2) -- (think2);
\draw[flow] (think2) -- (soap2);
\draw[flow] (soap2) -- (loss2);

% Weight transfer from Stage 1 to Stage 2
\draw[copyFlow] (qformer1.south) to[out=-100,in=90]
  node[pos=.56, right, note, text=oColor] {freeze + reuse\\Stage-1 weights} (qf2.north);

% ---------------------------------------------------------------------------
% Legend
% ---------------------------------------------------------------------------
\node[frozen, minimum width=16mm, minimum height=4.5mm, font=\tiny] at (0.75,0.45)
  {frozen};

\node[trainable, minimum width=16mm, minimum height=4.5mm, font=\tiny] at (2.35,0.45)
  {Q-Former};

\node[lora, minimum width=16mm, minimum height=4.5mm, font=\tiny] at (3.95,0.45)
  {LoRA thinker};

\node[loss, minimum width=16mm, minimum height=4.5mm, font=\tiny] at (5.65,0.45)
  {loss / target};

\draw[sFlow] (7.00,0.45) -- +(0.55,0)
  node[right, note, text=sColor] {Subjective path};

\draw[oFlow] (9.00,0.45) -- +(0.55,0)
  node[right, note, text=oColor] {Objective path};

\draw[apFlow] (11.00,0.45) -- +(0.55,0)
  node[right, note, text=apColor] {Assessment/Plan path};

\draw[conceptFlow] (13.55,0.45) -- +(0.55,0)
  node[right, note, text=conceptColor] {concept loss};

\node[anchor=east, note] at (17.55,0.45)
  {No diarization or role mask};

\end{tikzpicture}%
}
\caption{Improved overview of the two-stage Q-Former adaptation. Stage 1 expands the Q-Former into three SOAP-specialized query groups and shows the auxiliary section losses associated with each group. Stage 2 restores the native Qwen audio pathway and freezes the Stage-1 Q-Former.}
\label{fig:improved_qformer}
\end{figure*}
